$\infty$-jets of difeomorphisms preserving orbits of vector fields

Let $F$ be a smooth vector field defined in a neighborhood of the origin in $\mathbb{R}^n$, $F(O)=0$, and let $F_t$ be its local flow. Denote by $E$ the set of germs of diffeomorphisms $h:\mathbb{R}^n \to \mathbb{R}^n$ preserving orbits of $F$ and let $E_{\mathrm{id}}^r$ be the identity component of $E$ with respect to $C^r$-topology. Then every $E_{\mathrm{id}}^{r}$ contains a subset $Sh$ consisting of mappings of the form $F_{f(x)}(x)$, where $f: \mathbb{R}^n \to \mathbb{R}$ is a smooth function. It was proved earlier by the author that if $F$ is a linear vector field, then $Sh=E_{\mathrm{id}}^0$. In this paper we present a class of vector fields for which $Sh$ and $E_{\mathrm{id}}^1$ coincide on the level of $\infty$-jets. We also establish a parameter rigidity of linear vector fields and "reduced" Hamiltonian vector fields of real homogeneous polynomials in two variables.

==> intro.tex <==
\section{Introduction}\label{sect:intro}
Let $\BFld$ be a smooth ($C^{\infty}$) vector field on a smooth manifold $\Mman$ tangent to $\partial\Mman$, $\BFlow_t$ be the local flow generated by $\BFld$, $\singB$ the set of singular points of $\BFld$ which coicides with the set $\Fix\BFlow$ of fixed points of $\BFlow$, and $\Vman\subset\Mman$ be an open subset.

 In this paper we study the space of smooth mappings $\difM:\Vman\to\Mman$ preserving orbits of $\BFld$, i.e. $\difM(\Vman\cap \orb)\subset\orb$ for every orbit $\orb$ of $\BFld$.
 Our approach is based on the following idea.
 Since for every $x\in\Vman$ its image $\difM(x)$ belongs to the orbit of $\BFld$, we \emph{want to associate to $x$ the time $\sigma_{\difM}(x)$ between $x$ and $\difM(x)$ along the orbit $\orb_x$ of $x$}, so that 
\begin{equation}\label{equ:h_is_a_shift}
  \difM(x) = \BFlow_{\sigma_{\difM}(x)}(x).
\end{equation}
We will call $\sigma_{\difM}$ a shift-function for $\difM$, which in turn will be called the \emph{shift} along orbits of $\BFld$ via the function $\sigma_{\difM}$.

This idea were used in~\cite{EHoph:1937, Totoki:MFCKUS:1966, Kowada:JMSJ:1972} for study of reparametrizations of measure preserving flows.
In particular, it is allowed there that the identity~\eqref{equ:h_is_a_shift} holds only almost eveywhere, i.e. on a subset of a full measure, so $\sigma_{\difM}$ may be even discontinuous.
In contrast, we work in $C^{\infty}$-cathegory and require that \emph{$\sigma_{\difM}$ is $C^{\infty}$ provided so is $\difM$}.

In~\cite{Maks:TA:2003} the problem of finding representation~\eqref{equ:h_is_a_shift} were solved for linear flows.
In particular it was shown that if $\BFld$ is a linear vector field on $\RRR^n$, then for every diffeomorphism $\difM:\RRR^n\to\RRR^n$ preserving orbits of $\BFld$ and being isotopic to the identity map $\id_{\RRR^n}$ via orbit preserving isotopy there exists a $C^{\infty}$ shift-function $\sigma_{\difM}$.
Moreover, if a family $\difM_{s}$ of orbit preserving diffeomorphisms smoothly depends on some $k$-dimensional parameter $s$, then so does the family $\sigma_{\difM_s}$ of their shift-functions%
%%%%%%%%%%%%%%%%%%%%%%%%
\footnote[1]{
I must warn the reader that the paper~\cite{Maks:TA:2003} contains mistakes in estimations of continuity of the correspondence as a map $\difM\mapsto\sigma_{\difM}$ as a map between certain functional spaces.
Moreover these estimations were essentially used in~\cite{Maks:AGAG:2006} for the calculations of the homotopy types of stabilizers and orbits of Morse functions on surfaces.
We will repair the mistakes of~\cite{Maks:TA:2003} in another paper and show that in the situation  considered in~\cite{Maks:AGAG:2006} they reamin true.

Also notice that the formula~\cite[Eq.~(10)]{Maks:TA:2003} for the shift-function near a regular point is missprinted.
It must be read as follows:
$\alpha(x) = p_1 \circ \BFlow_{-a} \circ f(x) - p_1(x) + a$.
The consequences which were deduced from it in~\cite{Maks:TA:2003} remain true.
}.

%%%%%%%%%%%%%%%%%%%%%%%%
These two properties allow easily to establish a parameter rigidity of linear vector fields and even their \emph{regular extension}, see Theorem~\ref{th:param-rigid}.

Before formulating the results obtained in this paper, let us make some remarks concerning the obstructions for~\eqref{equ:h_is_a_shift}.


1. \emph{Evidently, $\sigma_{\difM}(z)$ is uniquely defined only if $z$ is non-periodic.
For a periodic point of a period $\theta$ the time $\sigma_{\difM}(z)$ is defined only up to a constant summand $n\theta$, $(n\in\ZZZ)$.
Moreover for a fixed point we can set $\sigma_{\difM}(z)$ to arbitrary number.}

This problem is often avoided by assuming that the set of periodic points is empty, e.g.~\cite[p.357]{Kowada:JMSJ:1972}.
Moreover, if we consider ergodic flows, then the set $\singB$  (as a non-trivial invarian subset) can be assummed to have measure $0$, whence the values of $\sigma_{\difM}$ on $\singB$ may be ignored.

2. \emph{If $z$ is a regular (even periodic) point of $\BFld$, then $\sigma_{\difM}$ can be smoothly defined near $z$}, see~\cite[\S3.1]{Maks:TA:2003} and footnote~1 for correct reading of ~\cite[Eq.~(10)]{Maks:TA:2003}.


3. \emph{Representation~\eqref{equ:h_sm_shift} implies that $\difM$ is homotopic to the identity embedding $i_{\Vman}:\Vman\subset\Mman$, e.g. via the following smooth orbit preserving homotopy $\difM_t(z)=\BFlow(z,t\sigma_{\difM}(z))$.}

4. Conversely, \emph{if we assume that $\difM$ is homotopic to $i_{\nbh}$ via orbit preseving homotopy, then (using this homotopy) we can smoothly define $\sigma_{\difM}$ on the set of regular points of $\BFld$ in $\nbh$, see~\cite[Th.~25]{Maks:TA:2003}, though it can be even discontinuous at fixed points.}

Actually $\sigma_{\difM}$ depends on a particular homotopy.
Moreover for some homotopy  $\sigma_{\difM}$ can be smooth at a singular point, but even discontinuous for another homotopy, see~\cite{Maks:partit}.
But if we suppose in addition that $\BFld$ is linear, then as noted above every $\sigma_{\difM}$ smoothly extends to all of $\nbh$, \cite[Th.~27, statement about (E)-point]{Maks:TA:2003}.

5. \emph{If $\sigma_{\difM}$ can be defined at some singular point $z$ of $\BFld$ so that it becomes smooth at $z$, then by~\cite[Cor.~21]{Maks:TA:2003} $\difM$ must be embedding at $z$}.


In this paper we consider the problem of solving~\eqref{equ:h_is_a_shift} in a small neighborhood $\Vman$ of a singular point of $\BFld$.
Our main result is an example of a class of vector fields for which~\eqref{equ:h_is_a_shift} can be defined on the level of $\jo{\infty}$-jets, i.e. for every $\difM$ as above we will find a smooth function $\sigma_{\difM}$ such that $\jo{\infty}$-jets of $\difM$ and the mapping $\BFlow_{\sigma_{\difM}}$ at $z$ coincide.

Together with results of~\cite{Maks:Hamvf:2006} this will give a full solution of~\eqref{equ:h_is_a_shift} for the case when $\BFld$ is a Hamiltonian vector field of a real homogeneous polynomial in two variables having no multiple factors.
In another paper the latter result will be used to extend calculations of~\cite{Maks:AGAG:2006} to a large class of functions on surfaces with degenerate singularities.

Now we start to formulate the results of this paper.

\subsection{Shift-map.}
Let $\BFld$ be a smooth vector field on a smooth manifold $\Mman$ tangent to $\partial\Mman$.
Then for every $x\in\Mman$ its orbit with respect to $\BFld$ is a unique map
$\orb_x: \RRR\supset(a_x,b_x) \to \Mman$ such that $\orb_x(0)=x$, $\dot{\orb}_x = \BFld(\orb_x)$, where $(a_x,b_x) \subset\RRR$ is the maximal interval on which such a map can be defined.
Then
$$
\BDom = \mathop\cup\limits_{x\in\Mman} x \times (a_x, b_x),
$$
is an open neighbourhood of $\Mman\times0$ in $\Mman\times\RRR$, and by definition the \emph{local flow\/} of $\BFld$ is the following map
$$\BFlow: \Mman\times\RRR \; \supset \;\BDom\longrightarrow\Mman,
\qquad
\BFlow(x,t) = \orb_x(t).
$$

For every open $\Vman \subset \Mman$ denote by $\funcBV$ the subset of $C^{\infty}(\Vman,\RRR)$ consisting of functions $\afunc$ whose graph $\Gamma_{\afunc}=\{(x,\afunc(x)) \ : \ x\in\Vman\}$ is included in $\BDom$.
Then $\funcBV$ is the maximal subset of $C^{\infty}(\Vman,\RRR)$ on which the following map
$$
\Shift: C^{\infty}(\Vman,\RRR) \supset  \funcBV \to C^{\infty}(\Vman,\Mman), \qquad
\Shift(\afunc)(x) = \BFlow(x,\afunc(x))
$$
is defined.
We will call $\Shift$ the \emph{shift-map} of $\BFld$ on $\Vman$ and denote its image in $C^{\infty}(\Vman,\Mman)$ by $\imShBV$.

%If $\Vman=\Mman$, then we abbreviate $\funcBV$ to $\funcB$ and $\imShBV$ to $\imShB$.

It is easy to see that $\Shift$ is $C^{r,r}_{W,W}$-continuous for all $r\geq 0$, i.e. it is conntinuous between the corresponding weak $C^{r}_{W}$ topologies of $\funcBV$ and $C^{\infty}(\Vman,\Mman)$, \cite[Lemma~2]{Maks:TA:2003}.
Moreover, if $\singB$ is nowhere dense in $\Vman$, then $\Shift$ is locally injective with respect to any $C^{r}_{W}$ topology of $\funcBV$, \cite[Prop.~14]{Maks:TA:2003}.


Denote by $\EBV$ the set of all smooth maps $\difM:\nbh\to\Mman$ such that
\begin{itemize}
\item
$\difM(\omega\cap\nbh)\subset\omega$ for every orbit $\omega$ of $\BFld$, in particular $\difM$ is fixed on $\singB\cap\Vman$ and
\item
$\difM$ is a local diffeomorphism at every $z\in\singB\cap\Vman$.
\end{itemize}
Let $\EidBVr{r}$, $(0\leq r\leq \infty)$, be the connected path-component of the identity embedding $i_{\Vman}:\Vman\subset\Mman$ in $\EndBV$ with respect to $C^{r}_{W}$-topology, see Section~\ref{defn:r-homotopies} for details.

Then we have the following inclusions:
\begin{equation}\label{equ:inclusions_sh_concmp}
\imShBV \subset \EidBVr{\infty} \subset\cdots\subset \EidBVr{1} \subset \EidBVr{0}.
\end{equation}

% % % % % % % % % % % % % % % % % % % % % % % % % 
Indeed, by~\cite[Corr.~21]{Maks:TA:2003}, $\imShBV \subset \EBV$ and for every $\afunc\in\funcBV$ the map $\Shift(\afunc)$ is $C^{\infty}$-homotopic to $i_{\Vman}$ in $\EBV$ via the following homotopy: $H_t(x)=\BFlow(x,t\afunc(x))$.
Hence $\imShBV \subset \EidBVr{\infty}$.
All other inclusions are evident.
% % % % % % % % % % % % % % % % % % % % % % % % % 



For every $z\in\Mman$ let $\FuncMz$ be the algebra of germs at $z$ of smooth functions $\Mman\to\RRR$, and $\DiffMz$ be the group of germs at $z$ of difffeomorphisms $(\Mman,z)\to(\Mman,z)$.

Suppose that $z\in\singB \cap \Vman$.
Then $\difM(z)=z$ for every $\difM\in\EBV$.
Moreover, as it was noted above the germ of $\difM$ at $z$ belongs to $\DiffMz$, so we have a natural projection
$$
g: \EBV \to \DiffMz,
$$
associating to every $\difM\in\EBV$ its germ at $z$.

Denote by $\gEBz$, $\gEIdBzr{r}$, $(0\geq r \geq \infty)$, and $\gimShBz$ the images of $\EBV$, $\EidBVr{r}$, and $\imShBV$ in $\DiffRno$ respectively.
Then $\gEBz$, $\gEIdBzr{r}$, and $\gimShBz$ are subgroups in $\DiffRno$ and similarly to~\eqref{equ:inclusions_sh_concmp} we have the inclusions:
$$ %\begin{equation}\label{equ:inclusions_sh_concmp}
\gimShBz \subset \gEIdBzr{\infty} \subset\cdots\subset \gEIdBzr{1} \subset \gEIdBzr{0}.
$$ %\end{equation}

%For every $k\geq 0$ denote by $\jo{k}\BFld$ the $k$-jet of $\BFld$ at $\orig$.
%Finally, choose local coordinates $(x_1,\ldots,x_n)$ at $z$ and define the map $$j^{\infty}:\DiffMz \to \RRR[[x_1,\ldots,x_n]]$$ associating to every $\difM\in\DiffMz$ its $j^{\infty}$-jet at $\orig$.

% 
% % 
% % 
% % Now let $z\in\singB$.
% % Then $\difM(z)=z$ for all 
% % 
% % Let $\DiffRno$ be the group of germs at $\orig$ of diffeomorphisms of $(\RRR^n,\orig)$.
% % Since $\BFld(\orig)=0$, it follows from definition that $\difM(\orig)=\orig$ for every $\difM\in\EBV$ and the germ of $\difM$ at $\orig$ is a diffeomorphism at $\orig$, so we have a natural projection
% % $$
% % g: \EBV \to \DiffRno,
% % $$
% % associating to every $\difM\in\EBV$ its germ at $\orig$.
% % Denote by $\gEndBz$, $\gEndIdBzr{r}$, $(0\geq r \geq \infty)$, and $\gimShB$ the images of $\EBV$, $\EidBVr{r}$, and $\imShBV$ in $\DiffRno$ respectively.
% % Then $\gEndBz$, $\gEndIdBzr{r}$, and $\gimShB$ are subgroups in $\DiffRno$.
% % 
% % %For every $k\geq 0$ denote by $\jo{k}\BFld$ the $k$-jet of $\BFld$ at $\orig$.
% % Let also $$j^{\infty}:\DiffRno \to \RRR[[x_1,\ldots,x_n]]$$ be the map associating to every $\difM\in\DiffRno$ its $j^{\infty}$-jet at $\orig$.
% % Then similarly to~\eqref{equ:inclusions_sh_concmp} we have the inclusions:
% % $$ %\begin{equation}\label{equ:inclusions_sh_concmp}
% % \gimShB \subset \gEndIdBzr{\infty} \subset\cdots\subset \gEndIdBzr{1} \subset \gEndIdBzr{0}.
% % $$ %\end{equation}
% 
% \section{Introduction}\label{sect:intro}
% Let $\BFld$ be a smooth ($C^{\infty}$) vector field on $\RRR^n$ such $\BFld(\orig)=0$.
% In this paper we study the group of orbit preserving diffeomorphisms of $\BFld$.
% 
% % % % % % % % % % % % % % % % % % 
% % Thus $\difM\in \EidBVr{r}$ if there exists a homotopy $\Hmap:\nbh\times I\to \RRR^n$ such that $\Hmap_0=i_{\Vman}:\Vman\subset\RRR^n$, $\Hmap_1=\difM$, $\Hmap_{t}\in\gEndBz$ for all $t\in I$, and all partial derivatives of $H$ in $x$ up to order $r$ continuously depend on $t$.
% % Such a homotopy will be called an \emph{$r$-homotopy}.
% % Thus $H$ can be regarded as a continuous path between $i_{\Vman}$ and $\difM$ in $\EndBV$ endowed with $C^{r}$ topology.
% % % % % % % % % % % % % % % % % % 
% 
% %It consists of all maps $\difM\in\EidBVr{r}$ which are $r$-homotopic to $i_{\Vman}$ in $\EBV$.
% %, see Section~\ref{sect:shift_map_image} for details.
% 
% % Consider the local flow $\BFlow$ of $\BFld$.
% % This is a map $$\BFlow: \RRR^n\times\RRR \supset \BDom\to\RRR^n$$
% % defined on certain open neighbourhood $\BDom$ of $\orig\times 0$ in $\RRR^n\times\RRR$.
% 
% Recall that for every $x\in\RRR^n$ its orbit with respect to $\BFld$ is a unique map
% $\orb_x: \RRR\supset(a_x,b_x) \to \RRR^n$ satisfying $\dot{\orb}_x = \BFld(\orb_x)$ and $\orb_x(0)=x$.
% The interval $(a_x,b_x) \subset\RRR$ is assumed to be maximal.
% Then 
% $$
% \BDom = \mathop\cup\limits_{x\in\RRR^n} x \times (a_x, b_x),
% $$
% is an open neighbourhood of $\RRR^n\times0$ in $\RRR^n\times\RRR$, and the \emph{local flow\/} of $\BFld$ is the following map
% $$\BFlow: \RRR^n\times\RRR \; \supset \;\BDom\longrightarrow\RRR^n,
% \qquad
% \BFlow(x,t) = \orb_x(t).
% $$
% 
% Let $\Vman$ be an open neighbourhood of $\orig$.
% Denote by $\funcBV$ the subset of $C^{\infty}(\Vman,\RRR)$ consisting of functions $\afunc$ whose graph $\Gamma_{\afunc}=\{(x,\afunc(x)) \ : \ x\in\Vman\}$ is included in $\BDom$.
% Then $\funcBV$ is the maximal subset of $C^{\infty}(\Vman,\RRR)$ on which the following map
% $$
% \Shift: C^{\infty}(\Vman,\RRR) \supset  \funcBV \to C^{\infty}(\Vman,\RRR^n), \qquad
% \Shift(\afunc)(x) = \BFlow(x,\afunc(x))
% $$
% is defined.
% We will call $\Shift$ the \emph{shift-map} of $\BFld$ on $\Vman$ and denote its image in $C^{\infty}(\Vman,\RRR^n)$ by $\imShBV$.
% 
% It is easy to see that $\Shift$ is $C^{r,r}_{W,W}$-continuous for all $r\geq 0$, i.e. it is conntinuous between the corresponding weak $C^{r}_{W}$ topologies of $\funcBV$ and $C^{\infty}(\Vman,\RRR^n)$, \cite[Lemma~2]{Maks:TA:2003}.
% Moreover, if $\singB$ is nowhere dense in $\Vman$, then $\Shift$ is locally injective with respect to any $C^{r}_{W}$ topology of $\funcBV$, \cite[Prop.~14]{Maks:TA:2003}.
% 
% 
% % 
% % Let also $\FuncRno$ be the algebra of germs at $\orig$ of smooth functions $\afunc:\RRR^n\to\RRR$.
% % Then we can define the following map
% % \begin{equation}\label{equ:local_shift_map}
% % \Shift: \FuncRno  \to \gEndBz, \qquad
% % \Shift(\afunc)(z) = \BFlow(z,\afunc(z)),
% % \end{equation}
% % which will be called the \emph{local shift-map} of $\BFld$ at $\orig$.
% % Denote the image of $\Shift$ by $\gimShB$.
% % By~\cite[Pr.~3]{Maks:TA:2003}, $\gimShB$ is a subgroup in $\gEndIdBz$.
% % 
% 
% Let $\singB$ be the set of singular points of $\BFld$.
% Denote by $\EBV$ the set of all smooth maps $\difM:\nbh\to\RRR^n$ such that
% \begin{itemize}
% \item
% $\difM(\omega\cap\nbh)\subset\omega$ for every orbit $\omega$ of $\BFld$, in particular $\difM$ is fixed on $\singB\cap\Vman$ and
% \item
% $\difM$ is a local diffeomorphism at every $z\in\singB\cap\Vman$.
% \end{itemize}
% Let $\EidBVr{r}$, $(0\leq r\leq \infty)$, be the connected path-component of the identity embedding $i_{\Vman}:\Vman\subset\RRR^n$ in $\EndBV$ with respect to $C^{r}_{W}$-topology, see Section~\ref{defn:r-homotopies} for details.
% 
% Then we have the following inclusions:
% \begin{equation}\label{equ:inclusions_sh_concmp}
% \imShBV \subset \EidBVr{\infty} \subset\cdots\subset \EidBVr{1} \subset \EidBVr{0}.
% \end{equation}
% 
% % % % % % % % % % % % % % % % % % % % % % % % % % 
% Indeed, by~\cite[Corr.~21]{Maks:TA:2003}, $\imShBV \subset \EBV$ and for every $\afunc\in\funcBV$ the map $\Shift(\afunc)$ is $C^{\infty}$-homotopic to $i_{\Vman}$ in $\EBV$ via the following homotopy: $H_t(x)=\BFlow(x,t\afunc(x))$.
% Hence $\imShBV \subset \EidBVr{\infty}$.
% All other inclusions are evident.
% % % % % % % % % % % % % % % % % % % % % % % % % % 

% 
% Let $\DiffRno$ be the group of germs at $\orig$ of diffeomorphisms of $(\RRR^n,\orig)$.
% Since $\BFld(\orig)=0$, it follows from definition that $\difM(\orig)=\orig$ for every $\difM\in\EBV$ and the germ of $\difM$ at $\orig$ is a diffeomorphism at $\orig$, so we have a natural projection
% $$
% g: \EBV \to \DiffRno,
% $$
% associating to every $\difM\in\EBV$ its germ at $\orig$.
% Denote by $\gEndBz$, $\gEndIdBzr{r}$, $(0\geq r \geq \infty)$, and $\gimShB$ the images of $\EBV$, $\EidBVr{r}$, and $\imShBV$ in $\DiffRno$ respectively.
% Then $\gEndBz$, $\gEndIdBzr{r}$, and $\gimShB$ are subgroups in $\DiffRno$.
% 
% %For every $k\geq 0$ denote by $\jo{k}\BFld$ the $k$-jet of $\BFld$ at $\orig$.
% Let also $$j^{\infty}:\DiffRno \to \RRR[[x_1,\ldots,x_n]]$$ be the map associating to every $\difM\in\DiffRno$ its $j^{\infty}$-jet at $\orig$.
% Then similarly to~\eqref{equ:inclusions_sh_concmp} we have the inclusions:
% $$ %\begin{equation}\label{equ:inclusions_sh_concmp}
% \gimShB \subset \gEndIdBzr{\infty} \subset\cdots\subset \gEndIdBzr{1} \subset \gEndIdBzr{0}.
% $$ %\end{equation}

%Then $\jo{\infty}\gimShB \subset \jo{\infty}\gEndIdBzr{\infty}$.

% Let also 
% 
% Indeed, if $\Shift(\afunc)$ at $\orig$ is $C^{\infty}$-isotopic to $\id$ via the following homotopy: $\BFlow(z,t\afunc(z))$.
% Hence $\gimShB \subset \gEndIdBzr{\infty}$.
% All other inclusions are evident.
% 
% Let $\BFld$ be a smooth ($C^{\infty}$) vector field on a near the origin $\orig\in\RRR^n$ such that $\BFld(\orig)=0$.
% In this paper we study the group $\gEndBz$ of germs at $\orig$ of $C^{\infty}$ diffeomorphisms $\difM:(\RRR^n,\orig)\to (\RRR^n,\orig)$ preserving orbits of $\BFld$.
% Thus $\difM\in\gEndBz$ provided there exists a neighbourhood $\nbh$ of $\orig$ such that $\difM(\orb\cap\nbh)\subset\orb$ for each orbit $\orb$ of $\BFld$.
% 
% Let also $\gEndIdBzr{r}$ be the ``identity component'' of $\gEndBz$ with respect to $C^{r}$-topology, $(0\leq r \leq \infty)$.
% More precisely $\difM\in\gEndIdBzr{r}$ provided there exists a neighbourhood $\nbh$ of $\orig$ and a homotopy $\Hmap:\nbh\times I\to \RRR^n$ such that $\Hmap_0=\id_{\RRR^n}$, $\Hmap_1=\difM$, $\Hmap_{t}\in\gEndBz$ for all $t\in I$, and all partial derivatives of $H$ in $x$ up to order $r$ continuously depend on $t$.
% Such a homotopy will be called a \emph{$r$-homotopy}.
% Thus $H$ can be regarded as a continuous path in $\gEndIdBz$ endowed $C^{r}$ topology.
% 
% Consider the local flow $\BFlow$ of $\BFld$.
% This is a map $$\BFlow: \RRR^n\times\RRR \supset \BDom\to\RRR^n$$
% defined on some open neighbourhood $\BDom$ of $\orig\times 0$ in $\RRR^n\times\RRR$.
% Let also $\FuncRno$ be the algebra of germs at $\orig$ of smooth functions $\afunc:\RRR^n\to\RRR$.
% Then we can define the following map
% \begin{equation}\label{equ:local_shift_map}
% \Shift: \FuncRno  \to \gEndBz, \qquad
% \Shift(\afunc)(z) = \BFlow(z,\afunc(z)),
% \end{equation}
% which will be called the \emph{shift-map} of $\BFld$ at $\orig$.
% Denote the image of $\Shift$ by $\gimShB$.
% By~\cite[Pr.~3]{Maks:TA:2003}, $\gimShB$ is a subgroup in $\gEndIdBz$.

%Let $\DiffRno$ be the group of germs at $\orig$ of diffeomorphisms of $(\RRR^n,\orig)$.
% Denote by $\gEndBz$ the subgroup $\DiffRno$ consisting of orbit preserving germs, i.e., $\difM\in\DiffRno$ belongs to $\gEndBz$ iff there exists a neighbourhood $\nbh$ of $\orig$ such that $\difM(\orb\cap\nbh)\subset\orb$ for each orbit $\orb$ of $\BFld$.


% Consider the local flow $\BFlow$ of $\BFld$.
% This is a map $\BFlow: \RRR^n\times\RRR \supset \BDom\to\RRR^n$ defined on some open neighbourhood $\BDom$ of $\orig\times 0$ in $\RRR^n\times\RRR$.
%Finally, let $C^{\infty}(\RRR^n,\orig)$ be the algebra of germs at $\orig$ of smooth functions $\afunc:\RRR^n\to\RRR$.
%Since $\BFld(\orig)=0$, the substitution of $\afunc$ into $\BFlow$ instead of time is correct and yields a well-defined germ of a map $(\RRR^n,\orig)\to(\RRR^n,\orig)$, see Lemma~\ref{lm:shift-types}.

% Notice that we have the following inclusions:
% $$
% \gimShB \subset \gEndIdBzr{\infty} \subset\cdots \subset \gEndIdBzr{1} \subset \gEndIdBzr{0}.
% $$
% Indeed, the germ $\Shift(\afunc)$ at $\orig$ is $C^{\infty}$-isotopic to $\id$ via the following homotopy: $\BFlow(z,t\afunc(z))$.
% Hence $\gimShB \subset \gEndIdBzr{\infty}$.
% All other inclusions are evident.
% 
% 
% 
% For every $k\geq 0$ denote by $\jo{k}\BFld$ the $k$-jet of $\BFld$ at $\orig$.
% Let also $$j^{\infty}:\gEndBz \to \RRR[[x_1,\ldots,x_n]]$$ be the map associating to every $\difM\in\gEndBz$ its $j^{\infty}$-jet at $\orig$.

In this paper we treat the following three problems.
%Positive answers to them imply parameter rigidity of a vector field and also allow to calculate homotopy types of 
\begin{question}[Internal description of the image of shift-map]\label{qu:Sh-id-comp}
Is it true that $\gimShBz=\gEIdBzr{r}$ for some $r$?
\end{question}

\begin{question}[Local sections of $\Shift$]\label{qu:local-sections}
Suppose that $\singB$ is nowhere dense in $\Mman$, so $\Shift$ is locally injective.
Is $\Shift$ a homeomorphism with respect to $C^{\infty}$ topologies?
Equivalently, whether local inverses of $\Shift$ are continuous with respect to $C^{\infty}$ topologies?
%In particular, does $\Shift$ satisfy path-lifting theorem?
\end{question}

%Another problem about lifting \emph{smooth}:

\begin{question}[``Smooth'' path-lifting theorem]\label{qu:lift-smooth-paths}
Let $\Hmap:\Vman\times I\to\Mman$ be an homotopy such that $\Hmap_t\in \imShBV$ for all $t\in I$, so $\Hmap_t(z)=\BFlow(z,\sigma_t(z))$ for some (perhaps not unique) smooth function $\sigma_t:\Vman\to\RRR$.
Thus we get a function $\sigma:\Vman\times I\to\RRR$ defined by $\sigma(z,t)=\sigma_t(z)$.
Suppose that $\Hmap$ is a $C^{\infty}$ map. 
Is it true that $\sigma$ can be chosen $C^{\infty}$ as well?
\end{question}


\begin{example}\label{exmp:lin_vf}\rm
In~\cite[Def.~24]{Maks:TA:2003} for every $k\geq0$ a certain ``extension'' property $(E)^k$ for a vector field was introduced.
It was proved that $(E)^0$ implies $\gimShBz = \gEIdBzr{0}$, see~\cite[Th.~25]{Maks:TA:2003}.
Moreover it can easily be seen that property $(E)^1$ implies smooth path-lifting theorem.

Suppose that $\BFld$ is a linear vector field, i.e., there exists a non-zero $(n\times n)$-matrix such that $\BFld(x)=Ax$ for all $x\in\RRR^n$, if we regard $\BFld$ as a map $\RRR^n\to\RRR^n$.
Then by~\cite[Th.~27, statement about (E)-point]{Maks:TA:2003} $\BFld$ has property $(E)^k$ for every $k\geq0$.
In particular, $\gimShBz = \gEIdBzr{0}$ and $\BFld$ smooth path-lifting theorem.
%Moreover, it also implies that smooth path-lifting theorem holds for $\BFld$ as well.
On the other hand, the answer to~\ref{qu:local-sections} is positive not for all matrices $A$.
\end{example}


\subsection{Parameter rigidity.}
In latter years there obtained many results concerning rigidity of hyperbolic and locally free actions of certain Lie groups and their latices, see e.g.~\cite{KatokSpatzier:PMIHES:1994,Hurder:CM:1994, Kanai:GAFA:1996,KatokSpatzier:TMIS:1997,Dajmanovic:LMD:2007,EinsiedlerFisher:IJM:2007} and references there.
Rigidity of an action $\afunc$ means that any action which is sufficiently close in a proper sense to $\afunc$ is conjugate to $\afunc$.

For instance, in a recent paper~\cite{Santos:ETDS:2007} by N.\;dos Santos a parameter rigidity of localy free action of a contractible Lie group on a closed manifold is studied.
In the case of vector fields, i.e. actions of $\RRR$, local freeness means regularity of orbits.
In contrast we will consider certain classes of vector fields with singular points, i.e. not locally free $\RRR$-actions, and prove their parameter rigidity, see Theorem~\ref{th:param-rigid} and Corollaries~\ref{cor:LinVF} and~\ref{cor:HamVF}.

%For simplicity we consider a local varaint.
\begin{definition}[Local parameter rigidity]\label{defn:param-rigid}{\rm (cf.~\cite{Santos:ETDS:2007})}
%Let $\BFld$ be a vector field in a neighborhood 
Say that a vector field $\BFld$ on $\Mman$ is {\bfseries parameter rigid at a point $z\in\Mman$} if for any germ of a vector field $\AFld$ at $z$ such that every orbit of $\AFld$ is included into some orbit of $\BFld$ there exists a germ at $z$ of $C^{\infty}$-function  $\afunc:\Mman\to\RRR$ such that $\AFld=\afunc \BFld$.
In other words, $\AFld$ is obtained from $\BFld$ by change of velocity.
\end{definition}
% The action is said to be cohomologically rigid if the first cohomologyof A is isomorphic to the first cohomology of the Lie algebra of G. It isparameter rigid if for each other action with the same orbit foliation,there is a smooth orbit-preserving diffeomorphism, isotopic throughsuch diffeomorphisms to the identity, which conjugates the action toa reparametrization of the other by an automorphism of G. 

Notice that $\singB\subset\singA$, so regular orbits of $\BFld$ may include singular points of $\AFld$ and in this case $\afunc$ vanishes at these points.
Also $\AFld$ be can be more degenerate than $\BFld$ on $\singB$.
On the other hand, outside the set $\singA$ of singular points of $\AFld$ vector fields $\BFld$ and $\AFld$ are parallel, and even there exists a germ of $C^{\infty}$ function $\afunc:\Mman\setminus\singA\to\RRR\setminus\{0\}$ such that $\AFld=\afunc \BFld$.
Definition~\ref{defn:param-rigid} requires that $\afunc$ smoothly extends to some neighbourhood of $\orig$.

%The changes of velocity of vector fields were considered e.g. in~\cite{Totoki:MFCKUS:1966,Kowada:JMSJ:1972,Parry:JLMS:1972}, but the multiplier function $\afunc$ is always assumed everywhere non-vanishing.
%That definition means that advantage of our result that we allow 

Evidently, if $\BFld(z)\not=0$, then $\BFld$ is parameter rigid at $z$.
Therefore the interesting case is when $\BFld(z)=0$.
The following theorem shows that positive answers to~\ref{qu:Sh-id-comp} and~\ref{qu:lift-smooth-paths} imply a parameter rigidity.
\begin{thParamRig} %\label{th:param-rigid}
%Let $\BFld$ be a vector field on $\Mman$.
If $\gimShBz=\gEIdBzr{\infty}$ and the shift-map $\Shift$ of $\BFld$ satisfies smooth path-lifting theorem, then $\BFld$ is parameter rigid at $\orig$.
\end{thParamRig}
As a corollary of results of~\cite{Maks:TA:2003}, see Example~\ref{exmp:lin_vf}, we get the following
\begin{corollary}\label{cor:LinVF}
Every linear vector field on $\RRR^n$ is parameter rigid at the origin $\orig$.
\end{corollary}
% This statement seems to be new inspite of the 
% I did not found such a result in available mathematical literature.



% \begin{proof}
% Let $\AFld$ be a vector field on $\Mman$ such that every orbit of $\AFld$ is included into some orbit of $\BFld$.
% It follows that $\EA \subset \EB$, whence $\EidAr{\infty} \subset \EidBr{\infty}=\imShB$.
% 
% Not loosing generality we can assume that $\AFld$ generates a global flow $\AFlow:\Mman\times\RRR\to\Mman$.
% Otherwise we can find a smooth everywhere positive function $\bfunc:\Mman\to(0,\infty)$ such that $\AFld_1=\bfunc\AFld$ generates a global flow.
% Then $\AFld$ and $\AFld_1$ has the same orbits.
% Moreover, if $\AFld_1=\afunc\BFld$ for some smooth function $\afunc:\Mman\to\RRR$, then $\AFld=\frac{\afunc}{\bfunc}\,\BFld$, where $\frac{\afunc}{\bfunc}$ is smooth on all of $\Mman$ as well.
% 
% Thus we have that $\AFlow_t\in\EidAr{\infty} \subset \imShB$ for all $t\in\RRR$.
% Since $\AFlow(x,t)$ is $C^{\infty}$ in $(x,t)$, it follows from smooth path-lifting property of $\BFld$ that there exists a smooth function $\sigma:\Mman\times \RRR$ such that $$\AFlow(x,t) = \BFlow(x,\sigma(x,t)).$$
% Moreover, as $\AFlow(x,0)=x$, we can assume that $\sigma(x,0)=0$ for all $x\in\Mman$.
% Differentiating both parts of this identity in $t$ and setting $t=0$ we get
% $$
% \AFld(x) = \frac{\partial \AFlow}{\partial t}(x,0) = 
% \frac{\partial \BFlow}{\partial t}(x,\sigma(x,t)) \cdot \sigma'_{t}(x,0) = 
% \BFld(x)\cdot \sigma'_{t}(x,0).
% $$
% It remains to put $\afunc(x) = \sigma'_{t}(x,0)$.
% \end{proof}


Now let $\BFld$ be a vector field on $\RRR^n$ such that $\BFld(\orig)=0$.
For every $k\geq 0$ denote by $\jo{k}\BFld$ the $k$-jet of $\BFld$ at $\orig$.
Define the following map $$j^{\infty}:\DiffMz \to \RRR[[x_1,\ldots,x_n]]$$ associating to every $\difM\in\DiffMz$ its $j^{\infty}$-jet at $\orig$.
We will introduce a certain condition \AST\ for the vector field $\BFld$, see Section~\ref{sect:prop-AST}, and prove the following result.


	
\begin{thAST}
% \begin{theorem}\label{th:AST_implies_infjets}
%Let $\BFld$ be a vector field on $\RRR^n$ and $\BFld(\orig)=0$.
If $\BFld$ has property \AST, then $$\jo{\infty}\gimShBO = \jo{\infty}\gEIdBOr{1}.$$
Moreover, for every $g\in \EidBVr{1}$ there exists a 
$C^{\dg}_{W}$-neighbourhood $\NN_{g}$ in $\EidBVr{1}$ and a map $\Omega:\NN_{g}\to C^{\infty}(\Vman,\RRR)$ being continuous with respect the corresponding $C^{\infty}$ topologies such that for every $\difM\in\NN_{g}$ 
$$ \jo{\infty}(\difM) = \jo{\infty}\bigl(\Shift(\Omega(\difM))\bigr), $$
where $\Shift(\Omega(\difM))(x) = \BFlow(x,\Omega(\difM)(x))$.
\end{thAST}
In other words, $\Shift$ has a section on the level of $\infty$-jets.

%\end{theorem}


% \begin{thAST}
% % \begin{theorem}\label{th:AST_implies_infjets}
% If $\BFld$ has property \AST, then $\jo{\infty}\gimShB = \jo{\infty}\gEndIdBzr{1}$.
% \end{thAST}

From this theorem and results of~\cite{Maks:Hamvf:2006,Maks:partit} we will get the following statement.

Let $\BFunc:\RRR^2\to\RRR$ be a real homogeneous polynomial in two variables without multiple factors.
Thus we can write
$$ %\begin{equation} \label{equ:decomp-for-Q}
\BFunc(x,y) = \prod_{i=1}^{l} L_i(x,y) \cdot \prod_{j=1}^{q} Q_j(x,y),
$$ %\end{equation}
where every $L_i$ is a linear function, every $Q_j$ is a definite (i.e. irreducible over $\RRR$) quadratic form, $L_i/L_{i'}\not=\mathrm{const}$ for $i\not=i'$, and $Q_j/Q_{j'}\not=\mathrm{const}$ for $j\not=j'$.
\begin{corollary}\label{cor:HamVF}
Let 
$\BFld= -\BFunc'_{y} \frac{\partial }{\partial x}  + \BFunc'_{x} \frac{\partial }{\partial y}$
be the Hamiltonian vector field of $g$.
If $l=0$ and $q\geq 2$, i.e., $g$ is a product of at least two distinct definite quadratic forms, then $\gimShBO=\gEIdBOr{1}$. % and $\imShBV=\EidBVr{1}$
In all other cases $\gimShBO = \gEIdBzr{0}$. % and $\imShBV=\EidBVr{0}$.

Let $\Vman$ be an open neighborhood of $\orig$.
Then for every $g\in\imShBV$ there exists a neighbourhood $\NN_{g}$ in $\imShBV$ and a $C^{\infty,\infty}_{W,W}$-continuous and respecting smoothness map $\Omega:\NN_{g}\to C^{\infty}(\Vman,\RRR)$ such that for every $\difM\in\NN_{g}$ 
$$ \difM(x)  =\Shift(\Omega(\difM))(x) = \BFlow(x,\Omega(\difM)(x)),$$
i.e. $\Shift$ has a continuous section.

In particular, $\BFld$ is parameter rigid.
\end{corollary}









\subsection{Structure of the paper.}
In Section~\ref{sect:param_rigidity} we prove Theorem~\ref{thParamRig}.
Sections~\ref{sect:prelim_lemmas} contains some preliminary statements concerning initial non-zero jets of smooth shift.
In Section~\ref{sect:main-res} we characterize subgroups $\grp$ of $\DiffRno$ which include $\gimShB$ and such that $\jo{\infty}\grp=\jo{\infty}\gimShB$.
In Section~\ref{sect:cont-corresp} we establish general result concerning $\jo{\infty}$-sections of shift-map.

Property \AST\ for the vector field is defined in Section~\ref{sect:prop-AST}.
Then in Section~\ref{sect:AST_implies_sh_e} we formulate the first statement 
Theorem~\ref{th:AST_implies_infjets}
Theorem~\ref{thAST} is proved in
prove describe subgroupps the main result concerning 


% 
% %Thus $\Shift$ has a \emph{real} continuous section.
% 
% % \begin{corollary}
% % Let $g:\RRR^2\to\RRR$ be a homogeneous polynomal of degree $\dg\geq2$ and $\BFld=(-g'_{y},g'_{x})$ be the Hamiltonian vector field of $g$.
% % If $g$ is a product
% % \end{corollary}
% 
% 
% 
% 
% %For every $k\geq 0$ denote by $\jo{k}\BFld$ the $k$-jet of $\BFld$ at $\orig$.
% 
% 
% % Let $\BFld$ be a smooth ($C^{\infty}$) vector field on a near the origin $\orig\in\RRR^n$ such that $\BFld(\orig)=0$.
% % In this paper we study the group $\gEndBz$ of germs at $\orig$ of $C^{\infty}$ diffeomorphisms $\difM:(\RRR^n,\orig)\to (\RRR^n,\orig)$ preserving orbits of $\BFld$.
% % Thus $\difM\in\gEndBz$ provided there exists a neighbourhood $\nbh$ of $\orig$ such that $\difM(\orb\cap\nbh)\subset\orb$ for each orbit $\orb$ of $\BFld$.
% % 
% %Our approach is based on the following idea.
% Let $\Mman$ be a smooth, connected, $m$-dimensional manifold, and $\BFld$ be a smooth vector field on $\Mman$.
% In this paper we study the group of orbit preserving diffeomorphisms of $\BFld$.
% 
% Our approach is based on the notion of smooth shifts along orbits of $\BFld$.
% % Notice that locally $\BFld$ can be regarded as an automous system of differential equations on $\Mman$ of the form $\dot x=\BFld(x)$.
% % Then for every $x\in\Mman$ denote by $\BFlow(x,t)$ the solution of this equation we can consider the \emph{maximal soulution\/} $\BFlow(x,t)$ 
% % % $\BFlow$ be the local flow of $\BFld$.
% % %
% Let $$\BFlow: \Mman\times\RRR \supset \BDom\longrightarrow\Mman$$ be the local flow of $\BFld$, where $\BDom$ is a certain open neighbourhood $\BDom$ of $\Mman\times 0$ in $\Mman\times\RRR$.
% If $\Mman$ is compact, then $\BDom=\Mman\times\RRR$.
% 
% %  such that 
% % for every fixed $x\in \Mman$ the curve $\BFlow(x,t)$ defined on open is an integral curve of $\BFld$.
% % This is a map with the following property
% % For every fixed $x\in \Mman$ the curve $\BFlow(x,t)$ defined on open is an integral curve of $\BFld$.
% % It is defined on some open neighbourhood $\BDom$ of $\Mman\times 0$ in $\Mman\times\RRR$ and satisfies the following conditions: $\BFlow(x,0)=x$ for all $x\in\Mman$, and $\BFlow(\BFlow(x,t),s)=\BFlow(x,s+t)$ provided $
% 
% 
% %Of coxurse, if $\Mman$ is compact, then $\BFlow$ is defined on all of $\Mman\times\RRR$.
% 
% Denote by $\singB$ the set of zeros of $\BFld$.
% Let also $\Vman\subset\Mman$ be an open subset, and $\difM:\Vman\to\Mman$ be a smooth map which preserves orbits of $\BFld$, i.e. $\difM(\orb\cap\Vman)\subset\orb$ for each orbit $\orb$ of $\BFld$.
% In particular $\difM$ is fixed on $\singB\cap\Vman$.
% 
% Thus for every $z\in\Vman$ its image $\difM(z)$ belongs to the orbit $\orb_{z}$ of $z$, and we
% \emph{want to associate to $z$ the time $\sigma_{\difM}(z)$ between $z$ and $\difM(z)$ along $\orb$} so thut 
% \begin{equation}\label{equ:h_sm_shift}
% \difM(z)=\BFlow(z,\sigma_{\difM}(z)).
% \end{equation}
% Such a function $\sigma_{\difM}:\Vman\to\RRR$ will be called a \emph{shift-function} for $\difM$, which in turn will be called the \emph{shift} along orbits of $\BFld$ via the function $\sigma_{\difM}$.
% 
% The ``ideal'' situation would be if $\sigma_{\difM}:\Vman\to\RRR$ were smooth as well as $\difM$.
% But in general this is not possible.
% There are certain obstructions to the existence of representation~\eqref{equ:h_sm_shift}.
% 
% 1. Evidently, $\sigma_{\difM}(z)$ is uniquely defined only if $z$ is non-periodic.
% For a periodic point of period $\theta$ the time $\sigma_{\difM}(z)$ is defined only up to a constant summand $n\theta$, $(n\in\ZZZ)$.
% Moreover for a fixed point we can set $\sigma_{\difM}(z)$ to arbitrary number.
% 
% 
% 2. If $\sigma_{\difM}$ can be defined at some singular point $z$ of $\BFld$ so that it becomes smooth at $z$, then by~\cite[Cor.~21]{Maks:TA:2003} $\difM$ must be embedding at $z$.
% 
% 3. Representation~\eqref{equ:h_sm_shift} implies that $\difM$ is homotopic to the identity embedding $i_{\Vman}:\Vman\subset\Mman$, e.g. via the following smooth orbit preserving homotopy $\difM_t(z)=\BFlow(z,t\sigma_{\difM}(z))$.
% 
% 4. Conversely, if we assume that $\difM$ is homotopic to $i_{\nbh}$ via orbit preseving homotopy, then (using this homotopy) we can smoothly define $\sigma_{\difM}$ on the set of regular points of $\BFld$ in $\nbh$, see~\cite[Th.~25]{Maks:TA:2003}, though it can be even discontinuous at fixed points.
% But if we suppose in addition that $\BFld$ is linear, then ~\cite[Th.~27, statement about (E)-point]{Maks:TA:2003} every $\sigma_{\difM}$ smoothly extends to all of $\nbh$.%
% %%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%
% \footnote{I must warn the reader that my paper~\cite{Maks:TA:2003} contains two mistakes in Th.~17 and Lm.~32.
% More precisely, all statements concerning continuity of local sections of shift-map, namely Definition~15 of ``section'' property (S), Theorems~1, 17, 27 (statement about (S)-point), and Lemmas~28, 32 should be changed.
% They will be corrected in a subsequent paper. 
% These mistakes make no influence on the results in the present paper.
% In particular, statement of ~\cite[Th.~27]{Maks:TA:2003} about ``extension'' property (E) which will be often referred remains true.
% 
% Moreover, unfortunately, the incorrect~\cite[Theorem~1]{Maks:TA:2003} was used in~\cite{Maks:AGAG:2006} for the description of stabilizers and orbits of Morse functions on surfaces.
% Nevertheless, in the situation considered in~\cite{Maks:AGAG:2006} this theorem remains true.
% }
% %%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% 
% 
% 5. On the other hand, there are examples of vector fields $\BFld$ on $\Mman=\RRR^2$, see~\cite{Maks:partit}, such that $\BFld(\orig)=0$ and if $\difM$ is an orbit preserving map which is only \emph{continuously} homotopic to $i_{\Vman}$ via an orbit preserving homotopy, i.e. there exists a continuous map $H:\nbh\times I\to\Mman$ such that $H_0=i_{\Vman}$, $H_1=\difM$, and $H_t:\nbh\to\Mman$ is a $C^{\infty}$ orbit preserving embedding, then $\sigma_{\difM}$ may be discontinuous at $\orig$.
% 
% These observations led to the following construction studied in~\cite{Maks:TA:2003} and which we will now adopt to non-global flows.
% Let $\funcBV$ be the subset of $C^{\infty}(\Vman,\RRR)$ consisting of functions $\afunc$ whose graph $\Gamma_{\afunc}=\{(x,\afunc(x)) \ : \ x\in\Vman\}$ is included in $\BDom$.
% Then $\funcBV$ is the maximal subset of $C^{\infty}(\Vman,\RRR)$ on which the following map
% $$
% \Shift: C^{\infty}(\Vman,\RRR) \supset  \funcBV \to C^{\infty}(\Mman,\Mman), \qquad
% \Shift(\afunc)(z) = \BFlow(z,\afunc(z))
% $$
% is defined.
% We will call $\Shift$ the \emph{shift-map} of $\BFld$ on $\Vman$ and will denote its image by $\imShBV$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\iffalse
%\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Thus $\EndIdBV$ consists of maps that are \emph{$1$-homotopic} to $i_{\Vman}$ in $\EndIdBV$, see Section~\ref{sect:intro}.

%The map $\Shift(\afunc)$ will also be denoted by $\Bsh{\afunc}$.
% ans is called the \emph{shift} along orbits of $\BFld$ via the function $\afunc$ which in turn will be called a \emph{shift-function} for $\Bsh{\afunc}$.


% 
%  be the algebra of germs at $\orig$ of smooth functions $\afunc:\RRR^n\to\RRR$.
% Then we can define the following map
% $$
% \Shift: C^{\infty}(\RRR^n,\orig)  \to \gEndBz, \qquad
% \Shift(\afunc)(z) = \BFlow(z,\afunc(z)).
% $$
% Since $\BFld(\orig)=0$, it follows from~\cite[Corollary~21]{Maks:TA:2003} that $\Shift$ is correctly defined.
% This map will be called the \emph{shift-map} of $\AFld$.
% Denote its image by $\gimShB$.
% Evidently, $$\gimShB \subset \gEndBz.$$
% %In orded to describe the set of all  Thus we can consider th
% It follows from~\cite[Pr.~14]{Maks:TA:2003} that $\Shift$ is \emph{locally injective} with respect to any $C^{r}$-topology of $C^{\infty}(\RRR^n,\orig)$.

% We are interesting in the following natural problems: internal description of the image $\imShB$ and existence of continuous local sections of $\ShB$, see %Sections~\ref{sect:shift_map_image}, \ref{sect:shift_map_inverses}, and 
% Question~\ref{qu:Sh-id-comp},~\ref{qu:local-sections}, and \ref{qu:lift-smooth-paths} below.
% It will be shown in Section~\ref{sect:param_rigidity} that positive answers to~\ref{qu:Sh-id-comp} and~\ref{qu:lift-smooth-paths} imply a \emph{parameter rigidity} of $\BFld$, see Theorem~\ref{defn:param-rigid}.
% 
% 
% Furhtermore, Theorem~\ref{defn:param-rigid} leads to Conjecture~\ref{conj:non-divisib} which roughly speaking claims that if $\BFld$ is a vector field defined on a small open neighbourhood $\Vman$ of a singular point $z$ of $\BFld$, then the non-divisibility of the initial non-zero jet $\jo{\dg}(\BFld,z)$ of $\BFld$ at $z$ implies that the above obstructions 2 and 3 are enough for an orbit preserving map $\difM$ to have a smooth shift-function $\sigma_{\difM}$ near $z$, i.e. when $\imShBV=\EidBVr{r}$ for some $r$. 
% 
% %The results of this paper give condition when the answers to questions above are
% Towards proving the conjecture we characterise the initial non-zero jets of maps $\difM\in\EidBVr{1}$ provided $\imShBV$ and $\EidBVr{1}$ coincide on the level of $\infty$-jets, see Theorem~\ref{th:main-equivalence-form}.
% Sections~\ref{sect:prf-lm:init-terms-flows}-\ref{sect:th-main-equiv} contain the proof of this theorem.
% 
% Moreover, using a variant of a well-known E.\;Borel's theorem, see Theorem~\ref{th:Borel}, we also prove that under conditions of~Theorem~\ref{th:main-equivalence-form} the shift-map has a continuous local section on the level of $\infty$-jets, see Theorem~\ref{th:cont-estimations}.
% Notice that Counterexample~\ref{c_exmp:non-resonant_flow} shows that the positive answer to Question~\ref{qu:lift-smooth-paths} does not imply in general the positive answer to Question~\ref{qu:local-sections}.
% But Theorem~\ref{th:main-equivalence-form} shows that nevertheless such an implication holds (in some sense) on the level of $\infty$-jets.
% 
% 
% The disadvantage of Theorem~\ref{th:main-equivalence-form} is that the conditions are given not in terms of $\BFld$ but in terms of the space $\EidBVr{1}$ itself.
% Nevertheless, in  Sections~\ref{sect:prop-AST}-\ref{sect:th:AST_implies_infjets} we describe a class of vector fields for which conditions of Theorem~\ref{th:main-equivalence-form} hold.


%Moreover, they would also allow to describe homotopy types of certain infinite-dimensional groups, see~\cite{Maks:AGAG:2006} in spite the mistakes in~\cite{Maks:TA:2003}.



% The paper arranged as follows.
% In Sections~\ref{sect:shift_map_image} and~\ref{sect:shift_map_inverses} we describe 
% 
% In Section~\ref{sect:param_rigidity} parameter rigidity 
% 
% Let $\BFld$ be a vector field defined in a neighbourhood of $\orig\in\RRR^n$.
% Suppose that %$\ord(\BFld)=\dg < \infty$, i.e. %\! -smallfor some $\dg\geq1$ we have that 
% $\jo{\dg-1}(\BFld)=0$ and 
% $$\PFunc = \jo{\dg}(\BFld):\RRR^n\to\RRR^n$$
% is a non-zero homogeneous map of degree $\dg$.
% For $\dg=1$ we will always write $$\PFunc(x) = \Lmatr\cdot x,$$ where $\Lmatr$ is a certain non-zero $n\times n$-matrix.


%\bigskip

%\section{The image of a shift-map}\label{sect:shift_map_image}


\section{Preliminaries}
Let $\nbh$ be an open subset of $\RRR^n$ and $f=(f_1,\ldots,f_m):\nbh\to\RRR^m$ be a smooth mapping.
For every compact $K\subset \nbh$ and $r\geq 0$ define the \emph{$r$-norm} of $f$ on $K$ by
$\|f\|^{r}_{K} =\sum\limits_{j=1}^{m} \sum\limits_{|i|\leq r} \sup\limits_{x\in K} |D^{i}f_j(x)|,$
where $i=(i_1,\ldots,i_n)$, $|i|=i_1+\cdots+i_n$, and
$D^i = \frac{\partial^{|i|}}{\partial x_1^{i_1}\cdots\partial x_{n}^{i_n}}.$
For a fixed $r$ the norms $\|f\|^{r}_{K}$ define the \emph{weak Whitney $C^{r}_{W}$ topology\/} on $C^{\infty}(\nbh,\RRR^m)$, see e.g.~\cite{GolubitskyGuillemin,Hirsch:DiffTop}.
A \emph{$C^{\infty}_{W}$-topology\/} on $C^{\infty}(\nbh,\RRR^m)$ is generated by $C^{r}_{W}$-topologies for all finite $r\geq0$.
\begin{definition}
Let $A,B,C,D$ be smooth manifolds, $\XX\subset C^{\infty}(A,B)$ and $\YY\subset C^{\infty}(C,D)$ two subsets, and $F:\XX\to\YY$ a map.
Say that $F$ is {\bfseries $C^{s,r}_{W,W}$-continuous} provided it is continuous from $C^{s}_{W}$-topology on $\XX$ to $C^{r}_{W}$-topology on $\YY$, $(r,s=0,1,\ldots,\infty)$.

Say that a map $G:A \to \YY$ is {\bfseries $C^{r}_{W}$-continuous\/} provided $G$ is continuous from the standard topology of $A$ to $C^{r}_{W}$-topology of $\YY$.

Similarly, a map $H:\YY \to A$ is {\bfseries $C^{r}_{W}$-continuous\/} provided $H$ is continuous from $C^{r}_{W}$-topology of $\YY$ to the standard topology of $A$.

A subset $\YY\subset C^{\infty}(C,D)$ is {\bfseries $C^{k}_{W}$-open\/} if it is open with respect to the induced  $C^{k}_{W}$-topology of $C^{\infty}(C,D)$.
\end{definition}

\begin{definition}\label{defn:r-homotopies}
%First we give the following definition.
Let $\Hmap:A\times I \to B$ be a homotopy such that for every $t\in I$ the mapping $\Hmap_t:A\to B$ is $C^{r}$.
We will call $\Hmap$ an {\bfseries $r$-homotopy} provided the following map
$$j^{r}\Hmap: A \times I \to J^{r}(A, B), 
\qquad (a,t) \mapsto j^{r}(\Hmap_t)(a),$$ 
associating to every $(a,t)$ the $r$-th jet of $\Hmap_t$ at $a$, is continuous.
In local coordinates this means that $\Hmap_t$ and all its partial derivatives along $A$ are continuous in $t$.
In particular, every $C^{r}$-homotopy is an $r$-homotopy as well.

Equivalently, regarding homotopy $\Hmap$ as a path $\hat\Hmap:I\to C^{\infty}(A,B)$, we see that $\Hmap$ is an {\bfseries $r$-homotopy} if and only if $\hat\Hmap$ is a continuous path to $C^{r}$-topology of $C^{\infty}(A,B)$.

If $\Hmap$ consists of embeddings it will be called an {\bfseries $r$-isotopy}.
\end{definition}

% Let $\nbh$ be a neighbourhood of $\orig$.
% A \emph{continuous} map $\Hmap=(\Hmap^1,\ldots,\Hmap^n): \nbh\times [0,1]\to \RRR^n$ such that $\Hmap_0=\id_{\RRR^n}$, $\Hmap_1=\difM$, $\Hmap_{t}\in\gEndBz$ for all $t\in [0,1]$, and every partial derivative 
% $$\frac{\partial \Hmap^i}{\partial x_j}(x_1,\ldots,x_n,t):\nbh\times [0,1]\to \RRR$$
% is continuous in $(x_1,\ldots,x_n,t)$.

% Turning to our vector field $\BFld$ denote by $\EBV$ the subset of $C^{\infty}(\Vman,\Mman)$ consisting of maps $\difM$ with the following properties:
% \begin{enumerate}
%  \item[\rm(i)]
% $\difM(\Vman\cap\orb)\subset\orb$ for every orbit $\orb$ of $\BFld$, in particular $\difM(z)=z$ for every singular point $z\in\singB$;
%  \item[\rm(ii)]
% $\difM$ is diffeomorphism at every $z\in\singB$;
% \end{enumerate}

In particular,  $\EidBVr{r}$ consists of all smooth maps $\difM:\Vman\to\Mman$ 

% Denote by $\EBV$ the set of all smooth mappings $\difM:\nbh\to\Mman$ such that
% \begin{itemize}
% \item
% $\difM(\omega\cap\nbh)\subset\omega$ for every orbit $\omega$ of $\BFld$, in particular $\difM$ is fixed on the set of singular points of $\BFld$ contained in $\nbh$;
% \item
% $\difM$ is a local diffeomorphism at every singular point of $\BFld$ in $\nbh$.
% \end{itemize}
% For every $r$, $(0\leq r\leq \infty)$ let $\EidBVr{r}$ be connected path-component of the identity embedding $i_{\Vman}:\Vman\subset\RRR^n$ in $\EndBV$ with respect to $C^{r}_{W}$-topology.
% It consists of all maps $\difM\in\EidBVr{r}$ which are $r$-homotopic to $i_{\Vman}$ in $\EBV$.
% %, see Section~\ref{sect:shift_map_image} for details.
% Then we have the following inclusions:
% \begin{equation}\label{equ:inclusions_sh_concmp}
% \imShBV \subset \EidBVr{\infty} \subset\cdots\subset \EidBVr{1} \subset \EidBVr{0}.
% \end{equation}
% The former one is the consequence of above obstructions 2 and 3.


%In particular, the connected path-component $\EidBVr{r}$ of the identity embedding $i_{\Vman}:\Vman\subset\Mman$ in $\EBV$ of maps $\difM$ that are $r$-homotopic in $\EBV$ to $i_{\Vman}$.

%  yTurning to our vector field $\BFld$ denote by $\EidBVr{r}$, $(0\leq r \leq \infty)$, the identity component of $\EBV$ with respect to the \emph{$C^{r}$ topology}.
% Thus $\EidBVr{r}$ consists  $i_{\Vman}:\Vman\subset\Mman$.
% Then we have the following inclusions:
% $$ %\begin{multline*}
% \imShBV \subset \EidBVr{\infty} \subset\cdots\subset \EidBVr{1} \subset \EidBVr{0}.
% $$ %\end{multline*}
% The former one follows from obstructions 2 and 3 described above.

% \begin{question}\label{qu:Sh-id-comp}
% Is it true that $\imShBV = \EidBVr{r}$ for some $r$?
% \end{question}
% It follows from~\eqref{equ:inclusions_sh_concmp} that the positive answer to~\ref{qu:Sh-id-comp} would imply that
% $$\imShBV = \EidBVr{\infty} = \cdots = \EidBVr{r}.$$
% 
% \begin{example}\rm
% By~\cite[statement of Th.~27 about (E)-point]{Maks:TA:2003} we have that $\imShBV = \EidBVr{0}$ for every linear vector field.
% %In particular, $\EidBVr{r} = \EidBVr{s}$ for all $r,s$.
% \end{example}
% \begin{example}\rm
% On the other hand, let $Q_1,\ldots,Q_{q}:\RRR^2\to\RRR$ be irreducible over $\RRR$ (definite) quadratic forms such that $Q_i/Q_j\not=\mathrm{const}$.
% Put $g=Q_1\cdots Q_{q}$ and let $\BFld=-g'_{y} \frac{\partial}{\partial x} + g'_{x} \frac{\partial}{\partial y}$ be the Hamiltonian vector field of $g$.
% Thus $\orig\in\RRR^2$ is a unique critical point of $g$ being its global extreme.
% The orbits of $\BFld$ are level sets $g^{-1}(c)$ of $g$.
% Every such orbit is either $\orig$ or a closed curve passing around $\orig$.
% It will follow from~\cite{Maks:Hamvf:2006,Maks:partit} and results of this paper that $\imShBV = \EidBVr{1} \subsetneq \EidBVr{0}$.
% \end{example}

% 
% \begin{example}\rm
% Let $g:\RRR^2\to\RRR$ be a real homogeneous polynomial without multiple factors, i.e., having no multuple complex roots.
% % 
% % On the other hand, let $Q_1,\ldots,Q_{q}:\RRR^2\to\RRR$ be irreducible over $\RRR$ (definite) quadratic forms such that $Q_i/Q_j\not=\mathrm{const}$.
% % Put $g=Q_1\cdots Q_{q}$ and 
% Let also $\BFld=-g'_{y} \frac{\partial}{\partial x} + g'_{x} \frac{\partial}{\partial y}$ be the Hamiltonian vector field of $g$.
% Then $\orig\in\RRR^2$ is a unique critical point of $g$ and the orbits of $\BFld$ are level sets $g^{-1}(c)$ of $g$.
% Every such an orbit is either $\orig$ or a closed curve passing around $\orig$.
% It follows from~\cite{Maks:Hamvf:2006,Maks:partit} and results of this paper that if $0$ is a degenerate extreme of $g$, i.e. $g$ is a product of at least two mutually non-proportional each to other irreducible over $\RRR$ quadratic forms, then $\imShBV = \EidBVr{1}$.
% In all other cases, $\imShBV = \EidBVr{0}$.
% \end{example}
% 

\section{Local sections of a shift-map}\label{sect:shift_map_inverses}


By~\cite[Lm.~14]{Maks:TA:2003} the shift-map $\Shift$ is $C^{r,r}_{W,W}$-continuous for all $r$.
Moreover it follows from~\cite[Pr.~14]{Maks:TA:2003} that $\Shift$ is \emph{locally injective} with respect to any $C^{r}$-topology of $C^{\infty}(\RRR^n,\orig)$ whenever $\singB$ is nowhere dense in $\Mman$.

Therefore it is natural to put the following:
%\item[\rm Q2]
%Since $\Shift$ is $C^{
%Since $\Shift$ is \emph{locally injective} with respect to any $C^{r}$-topology of $C^{\infty}(\RRR^n,\orig)$ it is natural to put the following two problems.
\begin{question}[Local sections of $\Shift$]\label{qu:local-sections}
Suppose that $\singB$ is nowhere dense in $\Mman$.
Whether $\Shift$ admits $C^{r,s}_{W,W}$-continuous local sections for some $s,r$? or at least for $r=s=\infty$?
%^with respect to some $C^{r}$ topologies?
In particular, does $\Shift$ satisfy path-lifting theorem?
\end{question}

%Another problem about lifting \emph{smooth}:

\begin{question}[``Smooth'' path-lifting theorem]\label{qu:lift-smooth-paths}
Let $\Hmap:\Vman\times I\to\Mman$ be an homotopy such that $\Hmap_t\in \imShBV$ for all $t\in I$, so $\Hmap_t(z)=\BFlow(z,\sigma_t(z))$ for some (perhaps not unique) smooth function $\sigma_t:\Vman\to\RRR$.
Thus we get a function $\sigma:\Vman\times I\to\RRR$ defined by $\sigma(z,t)=\sigma_t(z)$.
Suppose that $\Hmap$ is a $C^{\infty}$ map. 
Is it true that $\sigma$ can be chosen $C^{\infty}$ as well?
\end{question}


\begin{example}\rm
Let $\BFld$ be a linear vector field on $\RRR^n$, so $\BFld(z)=Az$ for some non-zero $(n\times n)$-matrix.
Then again it follows from~\cite[statement of Th.~27 about (E)-point]{Maks:TA:2003} that the answer to Question~\ref{qu:lift-smooth-paths} is {\bf yes}.
\end{example}
\begin{counterexample}\label{c_exmp:non-resonant_flow}
On the other hand there are matrices for which the answer to Question~\ref{qu:local-sections} is {\bf no} for any $r$.
Let 
$$
A = \mathrm{diag}\left[
\left(\begin{smallmatrix} 0 & \lambda_1 \\ -\lambda_1 & 0 \end{smallmatrix}\right),
\ldots,
\left(\begin{smallmatrix} 0 & \lambda_k \\ -\lambda_k & 0 \end{smallmatrix}\right),
0,\ldots,0
\right], \qquad \lambda_i\not=0, k\geq 2.
$$
In particular $n\geq 4$.
Suppose that there does not exist $\tau>0$ such that 
$$
\frac{\tau}{\lambda_i} \in \ZZZ, \qquad (i=1,\ldots,k).
$$
Then the shift-map $\Shift$ of $\BFld$ is injective.
% whibut a bijection with respect to all $C^{r}$-topologies of $C^{\infty}(\RRR^n,\RRR)$ and $\imShB$.
Its inverse %But the inverse map $\Shift^{-1}$ 
is not $C^{r,s}_{W,W}$-continuous for neither $r,s$.
This provided a counterexample to~\cite[Theorem~1]{Maks:TA:2003}.
\end{counterexample}
\begin{proof}
Represent $\RRR^n$ as $\CCC^{k}\times\RRR^{n-2k}$ and let $\nbh$ be an open neighbrourhood of $\orig$.
Then the flow of $\BFld$ is given by 
$$
\BFlow(z_1,\ldots,z_k,x) = (e^{i\lambda_1} z_1, \ldots, e^{i\lambda_k} z_1,x).
$$
%where $(z_1,\ldots,z_k,x)\in\CCC^{k}\times\RRR^{n-2k}$.
Thus every point $(0,\ldots,0,z_i,0,\ldots,0,x)$ with $z_i\not=0$ is periodic of period $\theta_i=\frac{2\pi}{\lambda_i}$.
Hence all non-fixed points of $\RRR^n$ are periodic for $\BFlow$ if and only if there exists $\tau>0$ such that
$$
\tau/\lambda_i \in \ZZZ, \qquad (i=1,\ldots,k).
$$
By assumption such $\tau$ does not exists.
Then every $z=(z_1,\ldots,z_k,x)$ with all non-zero $z_i$ is non-periodic and even recurrent.
In particular, $\BFld$ has non-closed orbits, whence by~\cite[Prop.~13 (2)]{Maks:TA:2003} the shift-map of the corresponding vector field $\BFld(z)=Az$ 
$$
\Shift:C^{\infty}(\Vman,\RRR)\to \imShB \subset C^{\infty}(\Vman,\RRR^n), 
\qquad
\Shift(\afunc)(z) = e^{A\afunc(z)} z
$$
is a $C^{r,r}_{W,W}$-continuous bijection for all $r$.
% Then every point $z=(z_1,\ldots,z_k,x)$ with all non-zero $z_i$ is non-periodic, whence the shift-map of $\BFld$ given by 
% $$
% \Shift(\afunc)(z) = e^{A\afunc(z)} z
% $$
% is a continuous bijection onto its image $\gEndIdBzr{0}$.
% We claim that $\Shift$ is not a homeomorphism with respect to any $C^r$-topologies.
%Let $\nbh$ be arbitrary compact neighbourhood of $\orig$.

Notice that for every $t\in\RRR$ regarded as a constant function the map $\Shift(t)=\BFlow_{t}$ is linear, whence its partial derivatives of order $r\geq2$ vanish.
Therefore for every compact subset $K\subset\nbh$ and $r\geq 2$ we have
$\|\BFlow_{t} - \id\|^{r}_{K} = \|\BFlow_{t} - \id\|^{1}_{K}$.
 
It follows from assumption on $\tau$ that there are arbitrary large $t$ such that the norm $\|\BFlow_{t} - \id\|^{1}_{K}$ is arbitrary small.
This implies that the image of arbitrary $C^{r}$-neighbourhood of zero-function $0:\RRR^n\to\RRR$ is not open in $\imShB$ in neither of $C^{s}$-topologies.
Therefore $\Shift^{-1}$ is not $C^{s,r}_{W,W}$-continuous at $i_{\Vman}$ for neither $r,s$.
\end{proof}


\subsection{Sections of $\Shift$ as cocylcles.}
Suppose that $\BFlow$ is a global flow.
Recall that a function $\SectShB:\Mman\times\RRR\to \RRR$ is called a \emph{cocycle\/} over the flow $\BFlow$
%,  or over the subgroup $T=\{\BFlow_{t}\} \subset \Diff(\Mman)$, 
provided
$$
\SectShB_{t+s}(x) = \SectShB_t(\BFlow_s(x)) + \SectShB_s(x).
$$
for all $x\in\Mman$ and $s,t\in\RRR$.
If in addition there exists a function $\afunc:\Mman\to\RRR$ such that 
$$
\SectShB(x,t) = \afunc(\BFlow_t(x))-\afunc(x),
$$
then a cocycle $\SectShB$ is called \emph{coboundary}.
%This type of cocycles is extensively studied, see e.g.~\cite{KeynesMaddenMarkleySears:review}

More generally, let $A$ be a group and $S$ be a semigroup with a unit element $e$.
Suppose that $S$ acts on $A$ from the right, i.e. there is a map $*:A\times S \to A$ such that $\afunc * e = \afunc$ and $\afunc *(\amap\,\bmap)=(\afunc*\amap)*\bmap$ for all $\afunc\in A$ and $\amap,\bmap\in S$.
Then the map $\SectShB:S\to A$ is called a \emph{cocycle} or a \emph{crossed homomorphism\/} with respect to action $*$ provided
$$
\SectShB(\amap\,\bmap) = ( \SectShB(\amap)*\bmap )\, \SectShB(\bmap).
$$
Similarly, $\SectShB$ is called a \emph{coboundary\/} if there exists $\afunc\in A$ such that $\SectShB(\amap)=(\afunc*\amap) \, \afunc^{-1}$.

Consider now the typical situation when the corresponding shift-map $\Shift:C^{\infty}(\Mman,\RRR)\to C^{\infty}(\Mman,\Mman)$ of $\BFld$ is injective.
%This is a typical situation.
For instance this holds if $\singB$ is nowhere dense and $\BFld$ has either at least one non-closed orbit or a singular point $z$ at which the linear part of $\BFld$ vanishes, i.e. $\jo{1}(\BFld)(z)=0$, \cite[Prop.~13]{Maks:TA:2003}.

Then by \cite[Eq~(8)]{Maks:TA:2003} the image $S = \imShB$ is a semigroup of $C^{\infty}(\Mman,\Mman)$ naturally acting on $A = C^{\infty}(\Mman,\RRR)$ from the right by composition:
$$
\afunc\circ \difM:\Mman \xrightarrow{s} \Mman \xrightarrow{\afunc} \RRR,
\qquad \afunc\in A, \, \difM \in S.
$$
Moreover, the same formula~\cite[Eq~(8)]{Maks:TA:2003} shows that the inverse map
$$
\SectShB=\Shift^{-1}:\imShB\to C^{\infty}(\Mman,\RRR)
$$
is a cocycle of this action, i.e. 
$$
\SectShB(\amap \circ \bmap) = \SectShB(\bmap) + \SectShB(\amap)\circ \bmap.
$$

Cocycles of flows or (semi-)group actions are useful in problems of reparametrizing the actions, see e.g.\! the introduction in~\cite{JTTY:MMJ:1997}.
There is %If $\Shift$ is not injective, then 
%Let us briefly compare this What can be said 

The first typical problem is whether a given cocycle represents a non-trivial cohomology class?

In general $\Shift^{-1}$ is not a coboundary.
, though in a neighbouyrIn a neighbourhood of a regular point $\Shift$ is a coboundary.
This follows from formula~\cite[Eq~(10)]{Maks:TA:2003} which unfortunately were incorrectly printed\footnote{Formula~\cite[Eq~(10)]{Maks:TA:2003} must be read as follows:
$\alpha(x) = p_1 \circ f \circ \Phi(x,-a) - p_1(x) + a$.}
In proper local coordinates in a neighbourhood of such a point the flow can be represented 
More precisely, a cocycle of a semigroup is called a \emph{coboundary} provided there exists 


The usual type of questions are the following: is a certain cocycle continuous or smooth? does it represent a non-trivial cohomology class?
They are similar to Questions~\ref{qu:local-sections} and~\ref{qu:lift-smooth-paths}.


Cocycles are usefull for study reparametrizing of flows, see e.g. the introduction in~\cite{JTTY:MMJ:1997}.
Moreover, they are used in proving rigidity results for actions of $\RRR^n$ or $\ZZZ^n$ or more generally lattices in Lie groups, see e.g.~\cite{Hurder:CM:1994, Kanai:GAFA:1996,KatokSpatzier:TMIS:1997,Santos:ETDS:2007} and references in these papers.
These papers mostly cocern locally free actions, so the corresponding foliations by orbits are regular.

In the case of flows, i.e. $\RRR$-actionsIn our case the We consider vector fielIn the next section we will show that if for our cocycle $\Shift^{-1}$ the answers to Questions~\ref{qu:local-sections} and~\ref{qu:Sh-id-comp} are affirmative, then the corresponding vector field has \emph{}

%There are many other types of cocycles associated to flows and more generally to actions of groups, see e.g.~\cite{TopDynProc:1995} for many reviews concerning distinc aspects of coomologies of group actions. 




\iffalse

First we recall the following definition.

In particular, a function $\SectShB:\Mman\times\RRR\to \RRR$ is called a \emph{cocycle} of the flow $\BFlow$, i.e. of the subgroup $T=\{\BFlow_{t}\}_{t\in\RRR}$ if
$$
\SectShB(x,t+s) = \SectShB(\BFlow(x,s),t) + \SectShB(x, s).
$$
This type of cocycles is extensively studied, see e.g.~\cite{}



This cocycle can be regarded as a ``thickening'' of the previous cocycle of $T$, i.e. we replace this group by the  
%\section{The inverse of a shift-map as a crossed homomorphisms.}

\begin{definition}
Let $A$ be a group and $S$ be a semigroup with a unit element $e$.
Then the {\bfseries right action} of $S$ on $A$ is a map $*:A\times S \to A$ such that $\afunc * e = \afunc$ and $\afunc *(\amap\,\bmap)=(\afunc*\amap)*\bmap$ for all $\afunc\in A$ and $\amap,\bmap\in S$.

A map $\SectShA:S\to A$ is called a {\bfseries crossed homomorphism} provided
$$
\SectShA(\amap\,\bmap) = ( \SectShA(\amap)*\bmap )\, \SectShA(\bmap).
$$
\end{definition}
Suppose that $\AFlow$ is global.
Put $A=\funcA=\Ci{\Mman}{\RRR}$ and $S=\im\ShA$.
Then $A$ is an abelian group and by~\cite[Eq~(8)]{Maks:Shifts} $S$ is a subsemigroup of $\Ci{\Mman}{\Mman}$ equipped with a natural right action $\circ$ on $A$ given by
$$
\afunc\circ s:\Mman \xrightarrow{s} \Mman \xrightarrow{\afunc} \RRR,
\qquad \afunc\in A, \, s\in S.
$$
Suppose that the shift-map $\ShA$ of $\AFlow$ is injective, i.e., $\ShA:\Ci{\Mman}{\RRR}\to\im\ShA$ is a bijection.
Then it follows from~\cite[Eq~(8)]{Maks:Shifts} that the inverse map 
$$
\SectShA=\ShA^{-1}:\im\ShA\to\Ci{\Mman}{\RRR}
$$
is a crossed homomorphism, i.e.
$$
\SectShA(\amap\circ\bmap) = \SectShA(\amap)\circ\bmap + \SectShA(\bmap), \qquad \forall \amap,\bmap\in S.
$$
If $\ShA$ is not injective, then the local inverse of $\ShA$ near $\id_{\Mman}$ is a \emph{local crossed homomorphism} in a natural sense which we are not going to describe.

Thus the problem 2) can be reformulated in the following way: \emph{whether the (local) crossed homomorphism $\ShA^{-1}$ is $\contSS{\infty}{\infty}$-continuous?}
This point of view on the shift-map will be considered in another paper.

%\subsection{Characterization of opennes of $\ShA$.}
%Let $\Vman \subset\Mman$ be a $\Dm$-submanifold and $\ShAV$ be the corresponding shift-map.
Notice that if $\im\ShA$ were a group and $\ShA^{-1}$ were a (local) homomorphism, then continuity of $\ShA^{-1}$ would be equivalent to its continuity at the unit element $\id_{\Mman}$ only, which of course is a simpler problem.
In our case $\im\ShA$ is just a semigroup, $\ShA^{-1}$ is a crossed homomorphism, and $\funcAV$ is in general an open subset of $\Ci{\Mman}{\RRR}$, i.e. a \emph{local} group.
Nevertheless we will now show that existence of continuous local inverses of $\ShA$ is equivalent to existence of a continuous local inverse at $\id_{\Mman}$.

%Suppose that $\Notice that local sections ofAnother point of view 
\fi



\section{Parametric rigidity}\label{sect:param_rigidity}
As a simple application we will now show that affirmative answers to Questions~\ref{qu:Sh-id-comp} and~\ref{qu:lift-smooth-paths} imply a parameter rigidity of $\BFld$.
%\subsection{}
\begin{definition}[Parametric rigidity of vector fields]\label{defn:param-rigid}
Say that a vector field $\BFld$ on $\Mman$ is {\bfseries parameter rigid} if for every vector field $\AFld$ such that every orbit of $\AFld$ is included into some orbit of $\BFld$ there exists a $C^{\infty}$-function $\afunc$ such that 
$\AFld=\afunc \BFld$.
\end{definition}

Notice that regular orbits of $\BFld$ may include singular points of $\AFld$ and in this case $\afunc$ vanishes at these points.
Moreover, outside the set $\singA$ of singular points of $\AFld$ vector fields $\BFld$ and $\AFld$ are parellel, and even there exists an everywhere non-zero $C^{\infty}$ function $\afunc:\Mman\setminus\singA\to\RRR$ such that $\AFld=\afunc \BFld$ on $\Mman\setminus\singA$.
Definition~\ref{defn:param-rigid} requires that $\afunc$ smoothly extends to all of $\Mman$.

\begin{theorem}\label{th:param-rigid}
Let $\BFld$ be a vector field on $\Mman$.
Suppose that the shift-map $\ShB$ of $\BFld$ satisfies smooth path-lifting theorem and $\imShB = \EidBr{\infty}$.
Then $\BFld$ is parameter rigid.
\end{theorem}
\begin{proof}
Let $\AFld$ be a vector field on $\Mman$ such that every orbit of $\AFld$ is included into some orbit of $\BFld$.
It follows that $\EA \subset \EB$, whence $\EidAr{\infty} \subset \EidBr{\infty}=\imShB$.

Not loosing generality we can assume that $\AFld$ generates a global flow $\AFlow:\Mman\times\RRR\to\Mman$.
Otherwise we can find a smooth everywhere positive function $\bfunc:\Mman\to(0,\infty)$ such that $\AFld_1=\bfunc\AFld$ generates a global flow.
Then $\AFld$ and $\AFld_1$ has the same orbits.
Moreover, if $\AFld_1=\afunc\BFld$ for some smooth function $\afunc:\Mman\to\RRR$, then $\AFld=\frac{\afunc}{\bfunc}\,\BFld$, where $\frac{\afunc}{\bfunc}$ is smooth on all of $\Mman$ as well.

Thus we have that $\AFlow_t\in\EidAr{\infty} \subset \imShB$ for all $t\in\RRR$.
Since $\AFlow(x,t)$ is $C^{\infty}$ in $(x,t)$, it follows from smooth path-lifting property of $\BFld$ that there exists a smooth function $\sigma:\Mman\times \RRR$ such that $$\AFlow(x,t) = \BFlow(x,\sigma(x,t)).$$
Moreover, as $\AFlow(x,0)=x$, we can assume that $\sigma(x,0)=0$ for all $x\in\Mman$.
Differentiating both parts of this identity in $t$ and setting $t=0$ we get
$$
\AFld(x) = \frac{\partial \AFlow}{\partial t}(x,0) = 
\frac{\partial \BFlow}{\partial t}(x,\sigma(x,t)) \cdot \sigma'_{t}(x,0) = 
\BFld(x)\cdot \sigma'_{t}(x,0).
$$
It remains to put $\afunc(x) = \sigma'_{t}(x,0)$.
\end{proof}



This result in particular shows that a vector field satisfying condition of this theorem is \emph{non-divisible by smooth functions} vanishing at some points.
Therefore it is natural to expect some conversion of this result.
Actually the following local Conjecture~\ref{conj:non-divisib} seems to be plausible.

% Let $\BFld$ be a smooth ($C^{\infty}$) vector field near the origin $\orig\in\RRR^n$ such that $\BFld(\orig)=0$.
%Roughly speaking the conjecture claims that if $\BFld$ is non-flat at $\orig$ and the first non-zero jet of $\BFld$ at $\orig$ (being a vector field with polynomial coordinate functions) is non-divisible by homogenoeus polynomials, then the answer to Question~\ref{qu:Sh-id-comp} for $\BFld$ is yes.
%We will give a necessary and sufficient condition for $\Bfld$ We will give 
%We will formulate its local variant.
%Let $\BFld$ be a smooth ($C^{\infty}$) vector field near the origin $\orig\in\RRR^n$ such that $\BFld(\orig)=0$.

Let $\BFld$ be a smooth ($C^{\infty}$) vector field near the origin $\orig\in\RRR^n$ such that $\BFld(\orig)=0$, and
$\BFlow: \RRR^n\times\RRR \supset \BDom\to\RRR^n$ be a local flow of $\BFld$.

Let $\DiffRno$ be the group of germs at $\orig$ of diffeomorphisms of $(\RRR^n,\orig)$.
Denote by $\gEndBz$ its subgroup consisting of orbit preserving germs, i.e., $\difM\in\gEndBz$ iff there exists a neighbourhood $\nbh$ of $\orig$ such that $\difM(\orb\cap\nbh)\subset\orb$ for each orbit $\orb$ of $\BFld$.

Let also $\gEndIdBzr{r}$ be the ``identity component'' of $\gEndBz$ with respect to $C^{r}$-topology, $(0\leq r \leq \infty)$.
More precisely $\difM\in\gEndIdBzr{r}$ provided there exists a neighbourhood $\nbh$ of $\orig$ and an $r$-homotopy $\Hmap:\nbh\times I\to \RRR^n$ such that $\Hmap_0=\id_{\RRR^n}$, $\Hmap_1=\difM$, $\Hmap_{t}\in\gEndBz$ for all $t\in I$.

% Consider the local flow $\BFlow$ of $\BFld$.
% This is a map $\BFlow: \RRR^n\times\RRR \supset \BDom\to\RRR^n$ defined on some open neighbourhood $\BDom$ of $\orig\times 0$ in $\RRR^n\times\RRR$.
Finally, let $C^{\infty}(\RRR^n,\orig)$ be the algebra of germs at $\orig$ of smooth functions $\afunc:\RRR^n\to\RRR$.
Then we can define the \emph{local shift-map} by
\begin{equation}\label{equ:local_shift_map}
\Shift: C^{\infty}(\RRR^n,\orig)  \to \gEndBz, \qquad
\Shift(\afunc)(z) = \BFlow(z,\afunc(z)).
\end{equation}
Since $\BFld(\orig)=0$, the substitution of $\afunc$ into $\BFlow$ instead of time is correct and yields a well-defined germ of a map $(\RRR^n,\orig)\to(\RRR^n,\orig)$, see Lemma~\ref{lm:shift-types}.

Denote the image of $\Shift$ by $\gimShB$.
By~\cite[Pr.~3]{Maks:TA:2003}, $\gimShB$ is a subgroup in $\gEndIdBz$.
Then we have the following inclusions:
$$
\gimShB \subset \gEndIdBzr{\infty} \subset\cdots \subset \gEndIdBzr{1} \subset \gEndIdBzr{0}.
$$
For every $k\geq 0$ denote by $\jo{k}\BFld$ the $k$-jet of $\BFld$ at $\orig$.
Let also $$j^{\infty}:\gEndBz \to \RRR[[x_1,\ldots,x_n]]$$ be the map associating to every $\difM\in\gEndBz$ its $j^{\infty}$-jet at $\orig$.
Then $\jo{\infty}\gimShB \subset \jo{\infty}\gEndIdBzr{\infty}$.

\begin{conjecture}\label{conj:non-divisib}
Suppose that there exists a finite $\dg\geq1$ such that $\jo{\dg-1}\BFld=0$, and $\jo{\dg}\BFld=\Qmap$ is a non-zero homogeneous vector field non-divisible by homogeneous polynomials, i.e., it can not be represented in the form $\Qmap=\omega\Pmap$, where $\omega$ is a homogeneous polynomial of degree $\deg\omega\geq1$ and $\Pmap$ is a homogeneous vector field.
Then $\gimShB=\gEndIdBzr{r}$ for some $r$.
\end{conjecture}

%We will give necessary and sufficient condition when $\gimShB$ coincides with $\gEndIdBzr{r}$ of the level of $\infty$-jets.

Put
$$
\gJShB = (\jo{\infty})^{-1} \bigl( \gimShB  \bigr).
$$
Then $\gJShB$ is a subset of $\DiffRno$ consisting of germs $\difM$ for which there exists a smooth function $\afunc\in C^{\infty}(\RRR^n,\orig)$ such that $\jo{\infty}(\difM) = \jo{\infty}(\Shift(\afunc))$.

Towards proving this conjecture, we will give a characterization of $\gJShB$ in terms of non-zero initial jets of its elements.


% give in this paper a necessary and sufficient condition on $\BFld$ when $\jo{\infty}\gimShB = \jo{\infty}\gEndIdBzr{1}$, see Theorem~\ref{th:main-equivalence-form}, i.e.\! when for every $\difM\in\gEndIdBzr{1}$ we can find a smooth function $\afunc$ such that $\infty$-jet of $\difM$ coincides with $\infty$-jet of the map $\Shift(\afunc)$.
% Actually this condition is given not in terms of $\BFld$ but in terms of $\gEndBz$ and therefore its verification is not so easy task.
% Nevertheless we are able to establish it for the case when $\BFld$ is completely integrable, see Section~\ref{sect:prop-AST}.
% 
% Finally, if this condition holds, then we are also able to affirmatively solve $\jo{\infty}$-analogues of other Questions~\ref{qu:local-sections} and~\ref{qu:lift-smooth-paths}, see Section~\ref{sect:Borel_th}.
% Therefore there is a chance, for non-flat vector fields with non-divisible initial jet to be parameter rigid.





% Towards proving this conjecture, we will give in this paper a necessary and sufficient condition on $\BFld$ when $\jo{\infty}\gimShB = \jo{\infty}\gEndIdBzr{1}$, see Theorem~\ref{th:main-equivalence-form}, i.e.\! when for every $\difM\in\gEndIdBzr{1}$ we can find a smooth function $\afunc$ such that $\infty$-jet of $\difM$ coincides with $\infty$-jet of the map $\Shift(\afunc)$.
% Actually this condition is given not in terms of $\BFld$ but in terms of $\gEndBz$ and therefore its verification is not so easy task.
% Nevertheless we are able to establish it for the case when $\BFld$ is completely integrable, see Section~\ref{sect:prop-AST}.
% 
% Finally, if this condition holds, then we are also able to affirmatively solve $\jo{\infty}$-analogues of other Questions~\ref{qu:local-sections} and~\ref{qu:lift-smooth-paths}, see Section~\ref{sect:Borel_th}.
% Therefore there is a chance, for non-flat vector fields with non-divisible initial jet to be parameter rigid.


% \subsection{Correctness of definition of local shift-map.}
% %For a smooth mapping $f:\RRR^n\to\RRR^m$ we will always 
% Let $C_{0}^{\infty}(\RRR^n,\RRR^n)$ be the space of germs at $\orig$ of smooth maps $f:\RRR^n\to\RRR^n$ such that $f(\orig)=\orig$.
% For $f\in C_{0}^{\infty}(\RRR^n,\RRR^n)$ denote by $\jo{k}(f)$ its $k$-jet at the origin $\orig\in\RRR^n$.
% The following lemma shows that for every function $\afunc\in C^{\infty}_{0}(\RRR^n,\RRR)$ the substitution of $\afunc$ into $\BFlow$ instead of time $t$ is correct.
% \begin{lemma}\label{lm:shift-types}
% For $\difM\in C_{0}^{\infty}(\RRR^n,\RRR^n)$ and $\afunc,\bfunc\in C^{\infty}_{0}(\RRR^n,\RRR)$ define the following two maps $\Bsh{\afunc},\hBshh{\bfunc}$ by
% $$
% \Bsh{\afunc}(x) = \BFlow(x,\afunc(x)),
% \qquad
% \hBshh{\bfunc}(x) = \BFlow(\difM(x),\bfunc(x)).
% $$
% If $\BFld(\orig)=0$, then the germs of $\Bsh{\afunc}$ and $\hBshh{\bfunc}$ are well-defined.
% Moreover, $\Bsh{\afunc}\in\gimShB$ is a germ of a diffeomorphism at $\orig$ and 
% \begin{equation}\label{equ:Bsh_hBsh_0}
% \Bsh{\afunc}^{-1} = \Bsh{-\afunc\circ \Bsh{\afunc}^{-1}}.
% \end{equation}
% If $\difM$ is a germ of a diffeomorphism, then so is $\hBshh{\bfunc}$ and 
% \begin{equation}\label{equ:Bsh_hBsh_1}
% \hBshh{\bfunc} = \Bsh{\bfunc\circ\difM^{-1}}\circ \difM.
% \end{equation}
% If $\difM\in\gEndIdBzr{r}$ for some $r$, $(0\leq r\leq \infty)$, then $\hBshh{\bfunc}\in\gEndIdBz$ as well.
% Finally,
% \begin{equation}\label{equ:Bsh_hBsh_4}
% \difM = \Bsh{\afunc} \qquad \Leftrightarrow \qquad \hBshh{-\afunc} = \id.
% \end{equation}
% \end{lemma}
% \begin{proof}
% First notice that the flow $\BFlow$ is defined only on some open neighbourhood $\BDom$ of $\orig\times0$ in $\RRR^n\times\RRR$.
% Therefore it is possible that the map $\Bsh{\afunc}$ and $\hBshh{\bfunc}$ are not globally defined.
% Nevertheless, if $\BFld(\orig)=0$, then for arbitrary large $A\geq0$ there exists a neighbourhood $W_{A}$ of $\orig$ such that $W_{A}\times[-A,A] \subset \BDom$.
% This is a standard result on dependence of solutions of ODE on initial values.
% 
% Hence if $A>|\afunc(0)|$ then $\Bsh{\afunc}$ is defined on some neighbourhood of $\orig$ included in $W_{A}$.
% The proof for $\hBshh{\bfunc}$ is similar.
% 
% Further, by~\cite[Corollary~21]{Maks:TA:2003} $\Bsh{\afunc}$ is a diffeomorphism at $\orig$, and \eqref{equ:Bsh_hBsh_0} follows from in \cite[Eq.(9)]{Maks:TA:2003}.
% 
% Eq.~\eqref{equ:Bsh_hBsh_1} just means that $\hBshh{\bfunc}(x) = \BFlow(\difM(x),\bfunc\circ\difM^{-1}\circ\difM(x))$.
% 
% Suppose that $\difM\in\gEndIdBzr{r}$ for some $r$, $(0\leq r\leq \infty)$.
% Then there exists a neighbourhood $\Vman$ of $\orig$ and an $r$-homotopy $H:\Vman\times I\to \RRR^{n}$ such that $H_0=i_{\Vman}$, $H_1=\difM$, $H_t\in\gEndIdBzr{r}$ for all $t\in I$.
% We can also assume that $\bfunc$ is defined on $\Vman$.
% Let $\mu:I\to I$ be a $C^{\infty}$-function such that $\mu[0,\frac{1}{3}]=0$, and $\mu[\frac{2}{3},1]=1$.
% Define the following map $H':\Vman\times I\to \RRR^n$ by
% $$
% H'(x,t) =\left\{
% \begin{array}{ll}
%  H(x,\mu(2t)), & t\in[0,\frac{1}{2}] \\[2mm]
%  \BFlow(x,\mu(2(t-\frac{1}{2})) \cdot \bfunc(x) ), & t\in[\frac{1}{2},1].
% \end{array}\right.
% $$
% Then it is easy to see that $H'$ is an $r$-homotopy between $i_{\Vman}$ and $\hBshh{\bfunc}$.
% Finally, the verification of~\eqref{equ:Bsh_hBsh_4} is direct. 
% \end{proof}


% In this paper we give necessary and sufficient condition on $\BFld$ when $\jo{\infty}\gimShB = \jo{\infty}\gEndIdBz$, see Theorem~\ref{th:main-equivalence-form}, i.e.\! when for every $\difM\in\gEndIdBz$ we can find a smooth function $\afunc$ such that $\infty$-jet of $\difM$ coincides with $\infty$-jet of the map $\Bsh{\afunc}$.
% 
% Moreover, in Section~\ref{sect:cont-corresp} we estimate continuity of this correspondence $\difM\mapsto\afunc$ using a well-known theorem of E.~Borel, see Section~\ref{sect:Borel_th}.
% 
% In Section~\ref{sect:prop-AST} we also present a class of vector fields satisfying this condition, see Theorem~\ref{th:AST_implies_infjets}.
% The applications will be given in another paper and we briefly describe them in Section~\ref{sect:apps}.

